Classifying Convex Bodies by their Contact and Intersection Graphs

Suppose that $A$ is a convex body in the plane and that $A_1,\dots,A_n$ are translates of $A$. Such translates give rise to an intersection graph of $A$, $G=(V,E)$, with vertices $V=\{1,\dots,n\}$ and edges $E=\{uv\mid A_u\cap A_v\neq \emptyset\}$. The subgraph $G'=(V, E')$ satisfying that $E'\subset E$ is the set of edges $uv$ for which the interiors of $A_u$ and $A_v$ are disjoint is a unit distance graph of $A$. If furthermore $G'=G$, i.e., if the interiors of $A_u$ and $A_v$ are disjoint whenever $u\neq v$, then $G$ is a contact graph of $A$. In this paper we study which pairs of convex bodies have the same contact, unit distance, or intersection graphs. We say that two convex bodies $A$ and $B$ are equivalent if there exists a linear transformation $B'$ of $B$ such that for any slope, the longest line segments with that slope contained in $A$ and $B'$, respectively, are equally long. For a broad class of convex bodies, including all strictly convex bodies and linear transformations of regular polygons, we show that the contact graphs of $A$ and $B$ are the same if and only if $A$ and $B$ are equivalent. We prove the same statement for unit distance and intersection graphs.

==> IntersectionApp.tex <==
\section{Proof of \Cref{lemma:realizeH}}\label{app:intersection}
Before we can prove \Cref{lemma:realizeH} we need to show some properties
of $Q^k_A$.

First we will show that in every drawing of $Q^k_A$ as an intersection graph, the cycle
$\alpha_k$ is contained in an annulus.
\begin{lemma}\label{lemma:annulus}
Let $X\in\{A,B\}$.
In any drawing of $Q^k_A$ as an intersection graph with respect to $X$, any $i\in[n]$, and any $j\in\{1,\ldots,k\}$, the vertex $v_i(j)$ is contained in the annulus $\setbuilder{x\in\R^2}{\norm{s_0x}{A}\in(2j-2,2j]}$.
Therefore, the cycle $\alpha_j$ is contained in the annulus $\setbuilder{x\in\R^2}{\norm{s_0x}{A}\in(2j-3,2j]}$.
\end{lemma}

\begin{proof}
The upper bound on $\norm{s_0v_i(j)}{X}$ holds as there is a path from $s_0$ to $v_i(j)$ consisting of only $j+1$ vertices.
For the lower bound, assume for contradiction that for some values of $i$ and $j$, there exists a drawing of $Q^k_A$ as an intersection graph where $\norm{s_0v_i(j)}{X}\leq 2j-2$.
We now claim that (i): $\left\lceil\frac{\norm{s_0u_j}{X}-2}{2}\right\rceil\leq d_j$ for all $j\in\{1,\ldots,k\}$ and (ii): $\left\lceil\frac{\norm{s_0u_i}{X}-2}{2}\right\rceil< d_i$. Together, (i) and (ii) contradict either the minimality of $(d_0,\ldots,d_{n-1})$ (if $X=A$) or the assumption from the remark after \Cref{const:Q}~(if $X=B$).

For part (i), note that since $\pi_j$ consists of $d_j+2$ vertices, we have $\norm{s_0u_j}{X}\leq 2(d_j+1)$, and it follows that $\left\lceil\frac{\norm{s_0u_j}{X}-2}{2}\right\rceil\leq \left\lceil d_j\right\rceil=d_j$.

For part (ii), note that since there is a path from $v_i(j)$ to $u_i$ consisting of $d_i-j+2$ vertices, we have $\norm{v_i(j)u_i}{X}\leq 2(d_i-j+1)$.
By the triangle inequality we now get
$\norm{s_0u_i}{X}\leq \norm{s_0v_i(j)}{X}+\norm{v_i(j)u_i}{X}\leq 2j-2+2(d_i-j+1)=2d_i$.
It now follows that $\left\lceil\frac{\norm{s_0u_i}{X}-2}{2}\right\rceil\leq\left\lceil\frac{2d_i-2}{2}\right\rceil=d_i-1<d_i$.
\end{proof}

We want to be able to conclude that two cycles $\alpha_k, \alpha'_k$ intersect
if the two annuli containing the cycles cross each other (as is also needed for
\Cref{lemma:edgesH}). This will be an easy consequence of the following lemma
which shows that the cycle $\alpha_k$ goes all the way around $s_0$ inside the annulus
in any drawing of $Q^k_A$ as an intersection graph.
\begin{lemma}\label{lemma:winding}
Let $X\in\{A,B\}$.
Consider any drawing of $Q_A^k$ as an intersection graph with respect to $X$ and any $j\in\{3,\ldots,k\}$, and consider $\alpha_j$ as a parameterized, closed curve $\alpha_j\colon [0,1]\longrightarrow \R^2$, such that for any $i\in[n]$, $\alpha_j$ interpolates linearly from $v_i(j)$ to $v_{i+1}(j)$ on the interval $[\frac{i}{n},\frac{i+1}{n}]$, where indices are taken modulo $n$.
We may then define a continuous argument function $\theta_{\alpha}\colon[0,1]\longrightarrow \R$ such that $\theta_{\alpha}(t)$ is an argument of the vector $\alpha_j(t)-s_0$ for all $t\in[0,1]$.
Then the argument variation of $\alpha_j$ around $s_0$ is $\theta_{\alpha}(1)-\theta_{\alpha}(0)=\pm 2\pi$.
\end{lemma}

\begin{proof}
Just as $\alpha_j$ is considered as a parameterized curve in the lemma, we may in a similar way consider $\sigma_{k'}$ as a parameterized closed curve $\mathcal \sigma_{k'}\colon [0,1]\longrightarrow \R^2$ such that $\sigma_{k'}$ interpolates linearly from $u_i$ to $u_{i+1}$ on the interval $[\frac{i}{n},\frac{i+1}{n}]$.
We also define $\theta_\sigma\colon[0,1]\longrightarrow\R$ to be a continuous argument function for $\sigma_{k'}$.
Since $\sigma_{k'}$ is a simple closed curve containing $s_0$ in the interior by Lemma~\ref{lemma:christmas}, we get that the argument variation of $\sigma_{k'}$ around $s_0$ is $\theta_\sigma(1)-\theta_\sigma(0)=2\pi$.

For any $\lambda\in[0,1]$, we now define the curve $\varphi_\lambda\colon[0,1]\longrightarrow\R^2$ such that $\varphi_\lambda(t)=(1-\lambda)\alpha_j(t)+\lambda \sigma_{k'}(t)$.
Thus, $\varphi_\lambda$ is a continuous interpolation between $\alpha_j$ (when $\lambda=0$) and $\sigma_{k'}$ (when $\lambda=1$).

We claim that for all $t,\lambda\in[0,1]$, we have $s_0\neq\varphi_\lambda(t)$.
To this end, we prove that the segment $\alpha_j(t)\sigma_{k'}(t)=\varphi_0(t)\varphi_1(t)$ is contained in the ball $D\mydef \setbuilder{x\in\R^2}{\norm{xu_i}{X}\leq \norm{\alpha_j(t)u_i}{X}}$, whereas $s_0\notin D$.

Suppose that $t=i/n+t'$, where $t'\in[0,\frac 1{2n})$.
The case where $t'\in[\frac 1{2n},\frac 1n)$ is similar.
We now have that
$$\norm{\alpha_j(t)u_i}{X}\leq
\norm{\alpha_j(t)v_i(j)}{X}+
\norm{v_i(j)u_i}{X}\leq
1+2(d_i-j+1)<2(d_i-1)+1<\norm{s_0u_i}{X},$$
so $s_0\notin D$.
Obviously, $\alpha_j(t)\in D$ by definition.
Since also $\norm{\sigma_{k'}(t)u_i}{X}\leq 1<\norm{s_0u_i}{X}$, the claim follows.

It now follows that for all $\lambda\in[0,1]$, the curve $\varphi_\lambda$ has the same argument variation around $s_0$ as $\sigma_{k'}$.
In particular, $\theta_{\alpha}(1)-\theta_{\alpha}(0)=\pm 2\pi$ as stated.
\end{proof}



\begin{figure}
\centering
\includegraphics{graphics/annulus.pdf}
\caption{Two cases from the proof of Lemma~\ref{lemma:realizeH}.}
\label{fig:annulus}
\end{figure}

% \begin{lemma}\label{lemma:realizeH}
%     Let $X\in\{A,B\}$ and $k\geq 7$.
%     In the setting of Lemma~\ref{lemma:edgesH}, consider an arbitrary drawing of $H_A^k(G)$ as in intersection graph with respect to $X$.
%     Then $\norm{s_0s'_0}{X}\geq 4k-18$ and if $ww'$ is an edge of $G$, then $\norm{s_0s'_0}{X}\leq 4k+2$.
% \end{lemma}

Now we have the tools available to prove \Cref{lemma:realizeH}.

\begin{proof}[Proof of \Cref{lemma:realizeH}]
    To prove the lower bound on $\norm{s_0s'_0}{X}$, we show that $\norm{s_0s'_0}{X}$ is neither in the interval $[0,k-7)$ nor in $[k-7,4k-18)$.
    The cases are depicted in Figure~\ref{fig:annulus}.
    \begin{enumerate}
    \item\label{lemma:realizeHcase1}
        Suppose that $\norm{s_0s'_0}{X}\in [0,k-7)$.
        Let $j\mydef \lceil\frac k2-2\rceil$.
        Then $s'_0$ is in the ball $s_0+(2j-3)X$.
        By Lemma~\ref{lemma:annulus}, $\alpha_j$ is contained in the annulus $\mathcal A\mydef \setbuilder{x\in\R^2}{\norm{s_0x}{X}\in (2j-3,2j]}$.
        Note that $\mathcal A$ has diameter $4j<2k-3$.
        It follows from Lemma~\ref{lemma:annulus} that any of the subpaths of $\pi'_{i'}$ from $s'_0$ to $v'_{i'}(k)$ connects the inner and outer boundary of $\mathcal A$.
        Therefore, Lemma~\ref{lemma:winding} gives that $\pi'_{i'}$ crosses $\alpha_j$.
        Thus, there is also an edge $v_i(j)v'_{i'}(j')$ of $H_A^k(G)$, where $j+j'\leq \lceil\frac k2-2\rceil+k<2k-4$, contradicting Lemma~\ref{lemma:edgesH}.
    
    \item\label{lemma:realizeHcase2}
        Suppose now that $\norm{s_0s'_0}{X}\in [k-7,4k-18)$.
        By an argument similar to the one used in the proof of Lemma~\ref{lemma:edgesH}, one can show that $\alpha_{k-3}$ crosses $\alpha'_{k-3}$.
        Hence, there is an edge $v_i(k-3)v'_{i'}(k-3)$, contradicting Lemma~\ref{lemma:edgesH}.
    \end{enumerate}
    
    Consider now the case that $ww'$ is an edge of $G$.
    By Lemma~\ref{lemma:edgesH}, we know that there is an edge $v_i(k)v'_{i'}(k)$.
    Then $\norm{s_0s'_0}{X}\leq \norm{s_0v_i(k)}{X}+\norm{v_i(k)v'_{i'}(k)}{X}+\norm{v'_{i'}(k)s'_0}{X}\leq 4k+2$.
\end{proof}
